TICO-19: the Translation Initiative for Covid-19

The COVID-19 pandemic is the worst pandemic to strike the world in over a century. Crucial to stemming the tide of the SARS-CoV-2 virus is communicating to vulnerable populations the means by which they can protect themselves. To this end, the collaborators forming the Translation Initiative for COvid-19 (TICO-19) have made test and development data available to AI and MT researchers in 35 different languages in order to foster the development of tools and resources for improving access to information about COVID-19 in these languages. In addition to 9 high-resourced, "pivot" languages, the team is targeting 26 lesser resourced languages, in particular languages of Africa, South Asia and South-East Asia, whose populations may be the most vulnerable to the spread of the virus. The same data is translated into all of the languages represented, meaning that testing or development can be done for any pairing of languages in the set. Further, the team is converting the test and development data into translation memories (TMXs) that can be used by localizers from and to any of the languages.

==> prev_intro_remain.tex <==

% In addition to 8 high-resourced, "pivot" languages---namely, Arabic, Chinese, French, Brazilian Portuguese, Latin American Spanish, Hindi, Russian, Swahili, Indonesian---the team is targeting 28 lesser resourced languages---namely, Bengali,  Burmese  (Myanmar), Farsi, Malay, Marathi, Tagalog, Tamil, Urdu, Dari, Central Khmer, Kurdish Kurmanji and Sorani, Nepali, Pashto, Amharic, Dinka, Nigerian Fulfulde, Kanuri, Kinyarwanda, Lingala, Luganda, Nuer, Oromo, Somali, Congolese Swahili, Tigrinya, Zulu. The latter set are primarily languages of of Africa, Asia and India, whose communities may be most susceptible to the spread of the virus and its potentially disastrous ramifications, due to lack of access to information and communication in the community languages. They are also overwhelmingly under-resourced languages; in fact, some of the languages have remained mostly untouched by the AI and MT communities, and have no known tools or resources that have been developed for them.

% The original source content (described in detail in Section~\ref{sec:benchmark}) is in English, derived from a variety of public sources containing COVID-19 related content. This data was then translated into all of the languages, in some cases, through pivot languages, i.e., the content was translated into the pivot language first (e.g., French, Farsi) and then translated into the target language (e.g., Congolese Swahili, Dari). All of the test and development documents are sentence aligned across all of the languages, which allows for any pairing of languages for testing or development purposes. This was done by design, in order to facilitate tool and resource development in and across any of the targeted languages. For example, an MT developer could develop translation systems for French to/from Congolese Swahili, Arabic to/from Kurdish, Urdu to/from Pashto, Hindi to/from Marathi, Amharic to/from Oromo, or Chinese to/from Malay (as examples among the 1296 possible pairings).

% Because of the breadth of languages covered by TICO-19, and the fact that so many are under-resourced, the translations themselves can be of significant value to localizers. As part of the effort, the TICO-19 collaborators have converted the translated data to translation memories, cast as TMX files, for all English--X pairings, as well as some other pairings of languages focusing on potential local needs (e.g. French--Kinyarwanda and Kurdish Kurmanji--Sorani). These TMX files, in addition to the test and development data itself, have been made available to the public.

Translators without Borders (TWB) worked with its network of translators to provide translations in hard to source languages (e.g. Congolese Swahili and Kanuri). It also provided COVID-19 specific sources from its diverse humanitarian partners to augment the dataset. This augmented dataset will be available under license on TWB's Gamayun portal\footnote{\url{https://gamayun.translatorswb.org/}}.

